CGHTRIMMER: Discretizing noisy Array CGH Data

The development of cancer is largely driven by the gain or loss of subsets of the genome, promoting uncontrolled growth or disabling defenses against it. Identifying genomic regions whose DNA copy number deviates from the normal is therefore central to understanding cancer evolution. Array-based comparative genomic hybridization (aCGH) is a high-throughput technique for identifying DNA gain or loss by quantifying total amounts of DNA matching defined probes relative to healthy diploid control samples. Due to the high level of noise in microarray data, however, interpretation of aCGH output is a difficult and error-prone task. In this work, we tackle the computational task of inferring the DNA copy number per genomic position from noisy aCGH data. We propose CGHTRIMMER, a novel segmentation method that uses a fast dynamic programming algorithm to solve for a least-squares objective function for copy number assignment. CGHTRIMMER consistently achieves superior precision and recall to leading competitors on benchmarks of synthetic data and real data from the Coriell cell lines. In addition, it finds several novel markers not recorded in the benchmarks but plausibly supported in the oncology literature. Furthermore, CGHTRIMMER achieves superior results with run-times from 1 to 3 orders of magnitude faster than its state-of-art competitors. CGHTRIMMER provides a new alternative for the problem of aCGH discretization that provides superior detection of fine-scale regions of gain or loss yet is fast enough to process very large data sets in seconds. It thus meets an important need for methods capable of handling the vast amounts of data being accumulated in high-throughput studies of tumor genetics.

==> makefile <==
RCSFLAGS= -l
MAIN= arxiv_trimmer
TEXPARTS= \
    000abstract.tex \
    010introduction.tex \
    030method.tex \
    040experiment.tex \
    050conclusion.tex \
    

BIBPARTS= BIB/*.bib
LPR = pspr # or change to 'qpr -q ps3'
POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
FIGPARTS = FIG/*.eps  FIG/*.pdf

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS)
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

#$(MAIN).pdf: $(MAIN).ps
#	ps2pdf $(MAIN).ps

#$(MAIN).ps: $(MAIN).dvi
#	$(POSTSCRIPT) -o $(MAIN).ps $(MAIN).dvi





#try: $(MAIN).tex
#	latex $(MAIN)

#$(MAIN).dvi: $(MAIN).tex $(TEXPARTS)
#	latex $(MAIN).tex
#	bibtex $(MAIN)
#	latex $(MAIN).tex
#	latex $(MAIN).tex
#	latex $(MAIN).tex

# print: $(MAIN).ps
# 	$(LPR) $(MAIN).ps

clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf

spotless: clean
	\rm -rf $(MAIN).ps $(MAIN).pdf
	\rm -rf TST

all.tar:
	tar cvfh all.tar makefile $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) README


